Write What You Want: Applying Text-to-video Retrieval to Audiovisual Archives

Audiovisual (AV) archives, as an essential reservoir of our cultural assets, are suffering from the issue of accessibility. The complex nature of the medium itself made processing and interaction an open challenge still in the field of computer vision, multimodal learning, and human-computer interaction, as well as in culture and heritage. In recent years, with the raising of video retrieval tasks, methods in retrieving video content with natural language (text-to-video retrieval) gained quite some attention and have reached a performance level where real-world application is on the horizon. Appealing as it may sound, such methods focus on retrieving videos using plain visual-focused descriptions of what has happened in the video and finding videos such as instructions. It is too early to say such methods would be the new paradigms for accessing and encoding complex video content into high-dimensional data, but they are indeed innovative attempts and foundations to build future exploratory interfaces for AV archives (e.g. allow users to write stories and retrieve related snippets in the archive, or encoding video content at high-level for visualisation). This work filled the application gap by examining such text-to-video retrieval methods from an implementation point of view and proposed and verified a classifier-enhanced workflow to allow better results when dealing with in-situ queries that might have been different from the training dataset. Such a workflow is then applied to the real-world archive from T\'el\'evision Suisse Romande (RTS) to create a demo. At last, a human-centred evaluation is conducted to understand whether the text-to-video retrieval methods improve the overall experience of accessing AV archives.

==> demoeval.tex <==
\section{Application and evaluation}
In the previous section, the proposed methods are proven to work as improvements to handle extra types of queries. However, the R@N indicator is purely a subjective quantitative measure for consistent performance evaluation across different models and methods. One of the main issues is that the testing ground truth is very strict and partial, where given a text query, only the single paired video is regarded as a success. This ignores the situation when sometimes the texts or videos are more or less similar, which, in human perception, is considered acceptable results. On the other hand, although in academia, text-to-video retrieval models have been tested and improved constantly with the standard datasets, seldom have they been applied to real-world archives. The ability of such models to support a satisfactory experience to explore the archive in the hope of gaining serendipitous findings is untested. To bridge these gaps, a demo retrieval system was built using the "MFT + Classifier" shown in table \ref{table:modelresult} with a subset of the RTS archive, and a human evaluation study was conducted.

\subsection{Data preparation}
\textbf{Dataset.}
Working with our content partner RTS, we have obtained an archive that covers a total of around 500,000 videos with total runtimes of around 150,000 hours and related production files, which takes up around 90 TB in storage. Although working with a real-world content partner is a privilege, the reality of RTS being a television station makes its content organised in different ways than traditional archives, with very limited content-related metadata. With these kinds of archives, such a text-to-video retrieval strategy would be the most appropriate and efficient way to open up the archive for the public, since it only requires a one-off encoding on the video end, and a large pre-trained model should already perform to a certain extent that no massive fine-tuning is needed. However, since the objective for this part is to provide a demo system for human evaluation, a subset of the whole archive is chosen and pre-processed for fine-tuning. For comprehensiveness and representativeness, a random batch of 100 videos with a total runtime of around 50 hours is used. Standard datasets used for Text-to-video retrieval tasks, take MSR-VTT as an example, has an average of 15 seconds in video runtime, and for each video, 20 corresponding textual descriptions are attached. It is clear that the real-world archive would require intensive pre-processing to be able to adapt to state-of-the-art encoding techniques.

\textbf{Video Segmentation.}
To produce video clips that are suitable for the proposed "MFT + Classifier" method, segmentation of the videos needs to be done first. Adaptive Content Detection in PySceneDetect\footnote{\url{https://github.com/Breakthrough/PySceneDetect}} is used for cutting the entire video. However, the method is adapted to only grayscale changes in a scene to avoid unnecessary cuts in long shots. Since the result clips vary in duration and can be really short, a 12 seconds threshold is set to group consecutive shot clips into a minimum of 12-second clips. As a result, a total of 7,348 short clips from 100 videos. Of which 70\% are less than 18 seconds. Fig.\ref{4} shows two segmentation results. In the first case (Video ZB015703), clip \#2 starts with a talking woman. At 00:00:06, there is a “jump cut” where the camera switch to another person. The detection method regards this moment as the end of this clip, but as this clip does not reach 12 seconds for now, we merge it with the subsequent clips until the total duration exceeds 12 seconds. The same situation also happens in clip \#3. The second case (Video ZX002510) has fast-moving scenes in some clips. The detection method is not sensitive to such scenes and does not cut them into shorter clips, preserving the completeness of the clips. 

\begin{figure}
    \centering 
    \includegraphics[width=.8\columnwidth]{4.png} 
    \caption{Segmentation results by adaptive content detection.}
\label{4}
\end{figure}

\textbf{Video Captioning.}
A newly available GPT-powered captioning model (\cite{tewel2022zero}) is tested but the issue of hallucinations of the GPT-powered ones introduce fictional elements to the content - after processing a video of two people chatting about a criminal case in an office, the model went on describing the actor's religion and race, which is not included in the video in any way. However interesting and useful these models can be for a generative purpose, it is not the most suitable for archival content description generation.
A dense captioning model, PDVC (\cite{wang2021end}), is used for generating descriptions of the video clips (Fig.\ref{5}). A random 1\% sample was collected and evaluated by a team of 3 annotators. Annotators were asked to reference the standard dataset samples from MSR-VTT and determine if the results from the captioning models are comparable or a failure. Annotator's evaluation yields an 83\% comparable rate, which is slightly lower than expected. However, considering many mistakes also occurring in the MSR-VTT dataset (such as grammar, spelling, and factual mistakes), we determined the quality of the generated captions usable. 80\% of these new caption and video pairs are used for fine-tuning the MFT model used in this demo phase. 
\begin{figure}
    \centering 
    \includegraphics[width=.8\columnwidth]{5.png} 
    \caption{Generated video descriptions examples by PDVC model.}
\label{5}
\end{figure}

\textbf{Text similarity.}
The dataset is then fed to Whisper to obtain transcripts for each video clip using the provided small model. Since a proportion of the language in the RTS archive is French, these transcripts are then translated into English with Helsinki-NLP/opus-mt-fr-en \footnote{\url{https://huggingface.co/Helsinki-NLP/opus-mt-fr-en}}. The final speech-to-text data obtained are stored in an ElasticSearch database for quote-related queries as mentioned in Section 3.3.


\subsection{Human evaluation}
The objective for the human evaluation part is two-fold. First, it evaluates whether the proposed "MFT + Classifier" method performs better compared to the original text-to-video retrieval models when handling more diverse queries (quote-related ones to be specific to this work). Second, it helps to understand whether the concept of applying text-to-video retrieval techniques to archives works and if the whole experience counts towards an improvement to the traditional keyword-based search. A total of 11 people
(5 male and 6 female, ages between 20 and 35) were recruited to do this evaluation. 
The experiment is designed in two stages. In the first stage, ten pre-defined visual and quote-related query pairs are used to retrieve video clips through MFT (trained on the original MSR-VTT and fine-tuned on the RTS caption-video pairs), as well as the proposed "MFT + Classifier" method. The top 3 results from each query and method were obtained and presented. The subject was asked to compare the results and to score them in a set order (see Fig\ref{6} for an example) and was instructed to evaluate the results by scoring on a 5-Likert scale. In the second stage, the query interface is open to the subject for a free exploration session using short narrative texts. Before the exploration, the subject is reminded of the limits of the demo caused by working on a small subset of the archive. At the end of the exploration, the subject is asked to vote between the given experience and their past experiences using other AV archive exploration interfaces (one of the typical archive explorative interface\footnote{\url{https://dc.library.northwestern.edu/}} is provided as reference). The subjects were required to conduct the overall evaluation based on the acute-eval metric \cite{li2019acute}, which emphasises the four key aspects when evaluating the performance and improvements of new methods and systems: Engagingness, Interestingness, Humanness, and Informativeness (relevance). 

\begin{table}[]
\begin{tabular}{cccc}
\hline
                 & Visual Queries & Quote-related Queries & Voting Against Other Systems \\ \hline
MFT              & 3.72           & 1.55                  & 6/11                         \\
MFT + Classifier & 3.64           & 4.64                  & 8/11                         \\ \hline
\end{tabular}

\caption{Results of human evaluation.}
\label{table:2}
\end{table}

\begin{figure}
    \centering 
    \includegraphics[width=.9\columnwidth]{6.png} 
    \caption{An example view of the evaluation interface. visual and quote-focused queries are presented at the top; method 1 represents the single MFT model, and method 2 represents the MFT + Classifier method.}
\label{6}
\end{figure}

The final evaluation results are reported in Table \ref{table:2}. The proposed "MFT + Classifier" method scored overall better than the single MFT model when handling more diverse queries. And regardless of the method deployed, more than half (6 and 8 out of 11 respectively) found the text-to-video retrieval as a strategy for exploring large AV archives better than a traditional keyword-based system.

